Attention-based Neural Cellular Automata

Recent extensions of Cellular Automata (CA) have incorporated key ideas from modern deep learning, dramatically extending their capabilities and catalyzing a new family of Neural Cellular Automata (NCA) techniques. Inspired by Transformer-based architectures, our work presents a new class of $\textit{attention-based}$ NCAs formed using a spatially localized$\unicode{x2014}$yet globally organized$\unicode{x2014}$self-attention scheme. We introduce an instance of this class named $\textit{Vision Transformer Cellular Automata}$ (ViTCA). We present quantitative and qualitative results on denoising autoencoding across six benchmark datasets, comparing ViTCA to a U-Net, a U-Net-based CA baseline (UNetCA), and a Vision Transformer (ViT). When comparing across architectures configured to similar parameter complexity, ViTCA architectures yield superior performance across all benchmarks and for nearly every evaluation metric. We present an ablation study on various architectural configurations of ViTCA, an analysis of its effect on cell states, and an investigation on its inductive biases. Finally, we examine its learned representations via linear probes on its converged cell state hidden representations, yielding, on average, superior results when compared to our U-Net, ViT, and UNetCA baselines.

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/abstract.tex <==
\begin{abstract}
   Recent extensions of Cellular Automata (CA) have incorporated key ideas from modern deep learning, dramatically extending their capabilities and catalyzing a new family of Neural Cellular Automata (NCA) techniques. Inspired by Transformer-based architectures, our work presents a new class of \textit{attention-based} NCAs formed using a spatially localized---yet globally organized---self-attention scheme. We introduce an instance of this class named \emph{Vision Transformer Cellular Automata (ViTCA)}. We present quantitative and qualitative results on denoising autoencoding across six benchmark datasets, comparing ViTCA to a U-Net, a U-Net-based CA baseline (UNetCA), and a Vision Transformer (ViT). When comparing across architectures configured to similar parameter complexity, ViTCA architectures yield superior performance across all benchmarks and for nearly every evaluation metric. We present an ablation study on various architectural configurations of ViTCA, an analysis of its effect on cell states, and an investigation on its inductive biases. Finally, we examine its learned representations via linear probes on its converged cell state hidden representations, yielding, on average, superior results when compared to our U-Net, ViT, and UNetCA baselines.
\end{abstract}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/acknowledgements.tex <==
\begin{ack}
First and foremost, M.\@T.\ thanks their former supervisor and mentor, Konstantinos (Kosta) G.\ Derpanis, for his invaluable support throughout the project.
M.\@T.\ also thanks Martin Weiss for his helpful feedback on implementing the linear probe experiments (\Sec{\ref{subsec:probing}});
Olexa Bilaniuk for his assistance in investigating the gradient differences caused by PyTorch's gradient checkpointing implementation (see Appendix \ref{subsec:extended_ablation}), and;
the Mila Innovation, Development, and Technology (IDT) team for their overall technical support, particularly, their tireless efforts maintaining cluster reliability during the crucial moments preceding the submission deadline.

M.\@T.\ is partially supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) Canada Graduate Scholarship -- Doctoral [application number CGSD3-519428-2018].
D.\@N.\ and C.\@P.\ are each partially supported by an NSERC Discovery Grant [application IDs 5011360 and 5018358, respectively]. D.\@N.\ thanks Samsung Electronics Co.\ Ldt.\ for their support. C.\@P.\ thanks CIFAR for their support under the AI Chairs Program.
\end{ack}
% thank kosta for his support throughout the project (e.g., he took time away from his family to video call and/or message with me almost every day during the holiday break to be my sounding board as I was trying to crack localized attention within an NCA on my whiteboard wall; since then, he consistently called me to see how I was doing and how the project was going while providing feedback on crucial questions pertaining to the intended contributions)
% thank Mila IDT for Mila cluster maintenance and uptime (in contrast, compute canada lost Narval during the few weeks prior to the neurips deadline, as well as an instable filesystem)
% thank Martin Weiss for his valuable feedback on implementing the linear probe experiments.
% thank Olexa for spending late hours into the night helping me debug PyTorch's gradient checkpointing implementation to figure out why there were differences in gradients when checkpointing vs not checkpointing

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/algorithms/vitca_training.tex <==
\begin{algorithm}[H]
    \label{alg:vitca_training}
    \caption{Training the ViTCA update rule with a ``pool sampling''-based approach}
    \Input{ViTCA cell update rule $F_\theta$, hyper-parameters $\Omega\!=\!$ $\{I\in\mathbb{N}^+,$ $b\in\mathbb{N}^+,$ $\sigma \in [0,1],$ $C_h \in \mathbb{N}^+,$ $\eta \in \mathbb{R}^+,$ $\alpha \in \mathbb{R},$ $\beta \in \mathbb{R},$ $N_\mathcal{P} \in\mathbb{N}^+\}$, dataset of images $\mathcal{D}\!=\!\{\mathbf{X}_1,\mathbf{X}_2,...,$ $\mathbf{X}_{N_b\in\mathbb{N}^+}\}$}
    \Output{Optimal update rule parameters $\theta_{I}$}
    $\theta_{0} \gets$ initial update rule parameters\Comment*[r]{\Eg He initialization \cite{he2015delving}}
    $\mathcal{P} \gets \emptyset$\Comment*[r]{Pool of cell grids and their respective ground truth images}
    \For{$i\gets1$ \KwTo $I$}{
        $\mathbf{X} \gets (\mathbf{X}_j,...,\mathbf{X}_{j+b})$ where $j \sim \mathcal{U}\{1,N_b-b\}$\Comment*[r]{$(\cdot,...,\cdot)$ is batch-wise concatenation}
        \eIf{$|\mathcal{P}| > b$ \and $i \bmod 2 = 0$}{
            $\mathbf{P} \gets \{(\mathbf{Z}_1,\mathbf{X}_1),..., (\mathbf{Z}_b,\mathbf{X}_b)\} \subset \mathcal{P}$\Comment*[r]{Retrieve first $b$ elements from the pool}
            $\mathbf{Z} \gets (\mathbf{Z}_1,...,\mathbf{Z}_b);\,\,\mathbf{X} \gets (\mathbf{X}_1,...,\mathbf{X}_b)$\Comment*[r]{Retrieve cell grids and images from $\mathbf{P}$}
        }{
            \Comment{Zero-initialize grids of cells and inject noisy inputs}
            \Comment{i is used for determining noise shape and coverage}
            \Comment{$C_h$ determines the number of cell hidden channels}
            $\mathbf{Z} \gets \texttt{seed}(\texttt{mask}(\mathbf{X}, i), C_h)$\;
        }
        $T \sim \mathcal{U}\{8,32\}$\Comment*[r]{Randomly sample number of cell updates to perform}
        \For{$t\gets1$ \KwTo $T$}{
            $\mathbf{Z} \gets F_{\theta_{i-1}}(\mathbf{Z}, \sigma)$\Comment*[r]{Iteratively update cell grids with cell update prob.\ $\sigma$}
        }
        \Comment{$\mathbf{Z}_o$ and $\mathbf{Z}_h$ are output and hidden channels of cell grids, respectively}
        $L_{o\_overflow} \gets \frac{1}{C_o}\|\mathbf{Z}_o-\min(\max(\mathbf{Z}_o, 0), 1)\|_1$\Comment*[r]{Output channels overflow loss}
        $L_{h\_overflow} \gets \frac{1}{C_h}\|\mathbf{Z}_h-\min(\max(\mathbf{Z}_h, -1), 1)\|_1$\Comment*[r]{Hidden channels overflow loss}
        $L_{rec} \gets \frac{1}{C_o}\|\mathbf{Z}_o - \mathbf{X}\|_1$\Comment*[r]{Image reconstruction loss}
        $L \gets \frac{1}{bHW}(\alpha L_{rec} + \beta(L_{o\_overflow} + L_{h\_overflow}))$\;
        $Q \gets \nabla L / (\|\nabla L\|_F + 10^{-8})$\Comment*[r]{Normalize gradients.\ $\|\cdot\|_F$ is Frob.\ norm}
        $\theta_i \gets \theta_{i-1} - \eta Q$\Comment*[r]{Update the update rule parameters}
        $\mathcal{P} \gets \mathcal{P} \cup \{(\mathbf{Z}_1,\mathbf{X}_1),...,(\mathbf{Z}_b,\mathbf{X}_b)\}$\Comment*[r]{Append updated cell grids and ground truths}
        $\mathcal{P} \gets \texttt{trunc}(\texttt{shuffle}(\mathcal{P}), N_\mathcal{P})$\Comment*[r]{Shuffle pool and retain first $N_\mathcal{P}$ elements}
    }
\end{algorithm}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{See \Sec{\ref{sec:discussion}}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Although we feel our work demonstrates the potential of NCAs as viable alternatives to common recurrent network architectures (ViTCA being our evidential contribution), our experiments intentionally tend towards the direction of optimizing model efficiency (and single-GPU training accessibility) rather than towards the increasingly popular direction of scaling upwards. However, as much as our work demonstrates the downward-scaling capabilities of NCAs, we also acknowledge that this similarly applies going upward, and as such, can be abused (\eg creating a ``deepfake''-capable ViTCA).}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code and instructions to reproduce results are included in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Given the combination of time and computational restrictions and our exhaustive list of experiments, we opted to prioritize experiment variety and dataset coverage as an implicit substitute for re-running experiments under different random seeds. For all experiments, we kept a fixed random seed, even pointing out (deterministic) differences caused by gradient checkpointing when used (see Appendix \ref{sec:appendix}).}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes
  \item Did you mention the license of the assets?
    \answerNA{Licensed frameworks used such as PyTorch (BSD-style) and Hydra (MIT) will be mentioned in acknowledgements.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{No new assets---aside from code and training our models---were created for the purposes of this work.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We used publicly available datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{Although not discussed in the manuscript, we would like to point that the datasets we used that could potentially contain personally identifiable information (CelebA, CIFAR10, Tiny ImageNet) each have restrictions and/or acknowledgements of such potential issues. Also, our work is not focused on classifying persons and ViTCA is not a generative model, \eg it can not generate new faces.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA
\end{enumerate}

\end{enumerate}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/discussion.tex <==
\vspace{-.5\baselineskip}
\section{Discussion}
\label{sec:discussion}
\vspace{-.5\baselineskip}
We have performed extensive quantitative and qualitative evaluations of our newly proposed ViTCA on a variety of datasets under a denoising autoencoding framework. We have demonstrated the superior denoising performance and robustness of our model when compared to a U-Net-based CA baseline (UNetCA) and ViT, as well as its generalization capabilities under a variety of environmental changes such as larger inputs (\ie spatial interpolation) and changing inputs \emph{during} cell updates.

Despite the computation savings---owed to our circumvention of self-attention's quadratic complexity by spatially localizing it within ViTCA---there remains the same memory limitations inherent to all recurrent models: multiple recurrent iterations are required for each training iteration, resulting in larger memory usage than a feedforward approach. This limits single-GPU training accessibility. We have experimented with gradient checkpointing \cite{chen2016training} but found its trade-off for increased backpropagation duration (and slightly different gradients) less than ideal. To fully realize the potential of NCAs (self-organization, inherent distributivity, \etc), we encourage follow-up work to address this limitation. Adapting recent techniques using implicit differentiation is one avenue to circumvent these issues~\cite{bai2022deep,bai2019deep}. Also, as mentioned in our ablation (\Sec{\ref{subsubsec:ablation_study}}), we hope to further investigate the instabilities caused by increasing the depth of ViTCA.
%
% Talk about potentially addressing the above limitation by using implicit differentiation, as inspired by DEQs, and talk about the difficulty in doing implicit diff the way DEQs does because of the stochastic cell update. Also talk about how I've had some promising results by doing the fixed-point solving only on the backward pass while retaining the usual CA stochastic update on the forward.
% Talk about investigating instability caused by increasing transformer depth and figuring out how to combine the benefits of increasing depth with the benefits of the CA recurrent update model.

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/equations/localize_attn.tex <==
\begin{tabular}{m{3.6in} c | m{1.25in}}
  \centering
  \vspace{-1.4\baselineskip}
  \begin{equation}
    \hspace{-1em}\mathbf{A}^{\!\star} = \texttt{softmax}{\left({\mathbf{A}^\prime}\big/{\sqrt{d}}\right)} \quad
    \st \left(\mathbf{A}^\prime\right)_{ij} = \sum_{l}(\mathbf{Q})_{il}(\mathbf{K})_{jl}
    \label{eq:localize_attn}
  \end{equation}
  \vspace{-1.4\baselineskip}
  & \text{\hspace{0.5em}} &
  \vspace{-1.4\baselineskip}
  \begin{equation}
    \sa^{\!\star} = \mathbf{A}^{\!\star}\mathbf{V}
    \label{eq:localized_attn}
  \end{equation}
  \vspace{-1.4\baselineskip}
\end{tabular}

with $\left( \mathbf{V} \right)_{jl}$ where $i\!=\!\{0,...,(N\!-\!1)\}$,  $j\!=\!\{(i+n_w+n_h),...,i,...,(i-n_w-n_h)\}$, and $l\!=\!\{0,...,(d-1)\}$, and with  $n_w\!=\!\{-\lfloor{N_W/2}\rfloor,...,0,...,\lfloor{N_W/2}\rfloor\}$ and  $n_h\!=\!\{-W\lfloor{N_H/2}\rfloor,...,0,...,W\lfloor{N_H/2}\rfloor\}$.

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/equations/losses.tex <==
\begin{equation}
  \begin{split}
    L_o &= \frac{1}{C_o}\|\mathbf{z}_o-\min(\max(\mathbf{z}_o, 0), 1)\|_1\ ,
    \\
    L_h &= \frac{1}{C_h}\|\mathbf{z}_h-\min(\max(\mathbf{z}_h, -1), 1)\|_1\ ,
    \\
    L_{rec} &= \frac{1}{C_o}\|\mathbf{z}_o - \mathbf{x}\|_1\ ,
    \\
    L &= \frac{1}{bHW}(\alpha L_{rec} + \beta(L_o + L_h))\ .
  \end{split}
  \label{eq:losses}
\end{equation}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/equations/sa.tex <==
\begin{tabular}{m{5.25in}}
  \centering
  \vspace{-1.4\baselineskip}
  \begin{equation}
    \hspace{0.08in}
    \sa = \texttt{softmax}{\left({\mathbf{QK}^T}\big/{\sqrt{d}}\right)\mathbf{V}}\ .
    \label{eq:sa}
  \end{equation}
  \vspace{-1.4\baselineskip}
\end{tabular}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/experiments.tex <==
\vspace{-.5\baselineskip}
\section{Experiments}
\vspace{-.5\baselineskip}
\label{sec:experiments}

Here we examine ViTCA through extensive experiments. We begin with experiments for denoising autoencoding, then an ablation study followed by various qualitative analyses, before concluding with linear probing experiments on the learned representations for MNIST \cite{deng2012mnist}, FashionMNIST \cite{xiao2017fashion}, and CIFAR10 \cite{krizhevsky2009learning}. We provide an extension to our experiments in Appendix \ref{sec:appendix}.

\paragraph{Baseline models and variants.}
% \textbf{Baseline models and variants.}
% Explain architecture construction for all models.
%  UNet: provide description similar to noise2noise's description and cite them. Point out how the number of pools has been reduced.
%  ViT: pe method, patch size, attention size, depth, embed dim, heads, head dim, mlp dim
%  ViTCA: same as ViT except attn size is 3x3. Include cell hidden dim.
%  UNetCA: modified version of UNet where init feats is 48 instead of 24 and all convs except first are changed to 1x1
%
Since we are performing pixel level reconstructions, we create a ViT baseline in which the class token has been removed. This applies identically for ViTCA. Unless otherwise stated, for our ViT and ViTCA models we use a patch size of $1\!\times\!1$ ($P_H\!=\!P_W\!=\!1$), and only a single encoding block with $h\!=\!4$ \mhsa\ heads, \embed\ size $d\!=\!128$, and \mlp\ size of $128$. For ViTCA, we choose $N_H\!=\!3$ and $N_W\!=\!3$ (\ie the \emph{Moore neighbourhood}~\cite{weissteinmoore}). We also compare with a U-Net baseline similar to the original formulation \cite{ronneberger2015u}, but based on the specific architecture from \cite{lehtinen2018noise2noise}. Since most of our datasets consist of $32\!\times\!32$ (resampled) images, we only have two downsampling steps as opposed to five. We implement a U-Net-based CA (UNetCA) baseline consisting of a modified version of our U-Net with 48 initial output feature maps as opposed to 24 and with all convolutions except the first changed to $1\!\times\!1$ to respect typical NCA restrictions~\cite{palm2022variational,mordvintsev2020growing}.

\vspace{-.5\baselineskip}
\subsection{Denoising autoencoding}
\vspace{-.5\baselineskip}
\label{subsec:denoising_autoencoding}
% Explain task and datasets used. Mention splits used for train, test, and val for each dataset.
% Optimizer, learning rate, learning rate schedule, batch size, number of training iterations, GPU used, loss function and scale factors, input/output size.
% Describe masking strategy and its scheduling. Describe how masking is performed during validation and test.

We compare between our baseline models and a number of ViTCA variants in the context of denoising autoencoding. We present test set results across six benchmark datasets: a land cover classification dataset intended for representation learning (LandCoverRep) \cite{yeh2021sustainbench}, MNIST, CelebA \cite{liu2015faceattributes}, FashionMNIST, CIFAR10, and Tiny ImageNet (a subset of ImageNet \cite{russakovsky2015imagenet}). All datasets consist of $32\!\times\!32$ resampled images except Tiny ImageNet, which is at $64\!\times\!64$ resolution. During testing, we use all masking combinations, chosen in a fixed order, and we update cells using a fixed number of iterations ($T\!=\!64$). See \Tab{\ref{tab:denoising_results}} for quantitative results.

Briefly mentioned in \Sec{\ref{subsec:update_rule}}, we employ a masking strategy inspired by Curriculum Learning (CL) \cite{wang2021survey,bengio2009curriculum} to ease training. This schedule follows a geometric progression of difficulty---tied to training iterations---maxing out at 10K training iterations. Specifically, masking starts at covering 25\% of the input with $1\!\times\!1$ patches of noise (dropout for RGB inputs, Gaussian for grayscale), then at each shift in difficulty, new masking configurations are added to the list of available masking configurations in the following order: $(2^0\!\times\!2^0, 50\%), (2^0\!\times\!2^0, 75\%), (2^1\!\times\!2^1, 25\%), (2^1\!\times\!2^1, 50\%), (2^1\!\times\!2^1, 75\%), ..., (2^2\!\times\!2^2, 75\%)$. Masking configurations are randomly chosen from this list.

We initialize weights/parameters using He initialization \cite{he2015delving}, except for the final layer of CA-based models, which are initialized to zero \cite{mordvintsev2020growing}. Unless otherwise stated, we train for $I\!=\!100$K iterations, use a minibatch size $b\!=\!32$, AdamW optimizer \cite{loshchilov2019decoupled}, learning rate $\eta\!=\!10^{-3}$ with a cosine annealing schedule \cite{loshchilov2017sgdr}, pool size \poolsize\ $\!=\!1024$, and cell hidden channel size $C_h\!=\!32$. In the case of Tiny ImageNet, $b\!=\!8$ to accommodate training on a single GPU (48GB Quadro RTX 8000). Training typically lasts a day at most, depending on the model. Due to the recurrent iterations required per training step, CA-based models take the longest to train. To alleviate memory limitations for some of our experiments, we use gradient checkpointing \cite{chen2016training} during CA iterations at the cost of backpropagation duration and slight variations in gradients due to its effect on round-off propagation. We also experiment with a cell fusion and mitosis scheme as an alternative. See Appendix \ref{sec:appendix} for details on runtime performance, gradient checkpointing, and fusion and mitosis.

\input{tables/denoising_results}

Amongst baselines, ViTCA outperforms on most metrics across the majority of datasets used (10 out of 18). Exceptions include LandCoverRep, where UNetCA universally outperforms by a small margin, likely due to the texture-dominant imagery being amenable to convolutions. Notably, ViTCA strongly outperforms on MNIST. Although MNIST is a trivial dataset for common tasks such as classification, our masking/noise strategy turns it into a challenging dataset for denoising autoencoding, \eg it is difficult for even a human to classify a $32\!\times\!32$ MNIST digit 75\% corrupted by $4\!\times\!4$ patches of Gaussian noise. We hypothesize that when compared to convolutional models, ViTCA's weaker inductive biases (owed to attention \cite{yifan2021input,jaegle2021perceiver}) immediately outperform these models when there are large regions lacking useful features, \eg MNIST digits cover a small space in the canvas. This is not the case with FashionMNIST, where the content is more filled out. Between baselines and ViTCA variants, ViTCA-32 (32 heads) and 32xy (xy-coordinate positional encoding) outperform all models by large margins, demonstrating the benefits of multi-head self-attention. We also experiment with a parameter-reduced (by $\sim\!60\%$), inverted bottleneck variant where $d\!=\!64$ and \mlp\ size is 256, often with a minimal reduction in performance.
%
%\paragraph{Training on high-resolution imagery.}
%\lipsum[4]
% Could go in appendix
% Talk about alternative approach to checkpointing to save memory by doing cell fusion/mitosis. Mention how this can be interpreted as being analagous to how Perceiver IO does sequence length compression to perform bulk of computations before uncompressing back to original length.
% Don't have final results but just say that results were promising and validation errors were not much higher while saving up to 50% memory and > 1 order of magnitude faster. This is something left for future work.
% \newpage
\vspace{-.5\baselineskip}
\subsubsection{Ablation study}
\label{subsubsec:ablation_study}
\vspace{-.5\baselineskip}
% Ablations only apply to baseline model, although do mention ablations on variant models when deemed necessary.
% \input{tables/ablation_results}

In \Tab{\ref{tab:ablation_results}} we perform an ablation study using the baseline ViTCA model above as reference on CelebA. Results are ordered in row-wise blocks, top-to-bottom. Specifically, we examine the impact of varying the cell hidden size $C_h$; the \embed\ size $d$; the number of \mhsa\ heads $h$; the depth (\# encoders), comparing both ViTCA (used throughout the table) with ViT; and in the last block we examine the impact of various methods of incorporating positional information into the model.

\input{tables/ablation_results}

Specifically, we examine the use of: (1) a xy-coordinate-based positional encoding \emph{concatenated} (``injected'') to cells, and; (2) a Transformer-based positional encoding (or embedding, if learned) \emph{added} into \embed. These two categories are subdivided into: 
(1a) sincos5---consisting of handcrafted Fourier features \cite{mildenhall2020nerf} with four doublings of a base frequency, \ie \pe\ $\!=\!(\sin{2^0\pi p},$ $\cos{2^0\pi p},$ $...,\sin{2^{J-1}\pi p},$ $\cos{2^{J-1}\pi p})\!\in\mathbb{R}^{N \times (4JP_HP_W)}$ where $J\!=\!5$ and $p$ is the pixel coordinate (normalized to [-1,1]) for each pixel the cell is situated on (one pixel since $P_H\!=\!P_W\!=\!1$); 
(1b) sincos5xy---consisting of both Fourier features and explicit xy-coordinates concatenated; 
(1c) xy---only xy-coordinates; 
(2a) handcrafted (our baseline approach)---sinusoidal encoding \pe\ $\!\in\!\mathbb{R}^{N \times d}$ similar to (1a) but following a Transformer-based approach \cite{vaswani2017attention}, and; 
(2b) learned---learned embedding \pe\ $\!\in\!\mathbb{R}^{N \times d}$ following the original ViT approach \cite{dosovitskiy2020image}. 
To further test the self-organizing capabilities of ViTCA, we also include: (3) none---no explicit positioning provided, where we let the cells localize themselves.

As shown in \Tab{\ref{tab:ablation_results}}, ViTCA benefits from an increase to most CA and Transformer-centric parameters, at the cost of computational complexity and/or an increase in parameter count. A noticeable decrease in performance is observed when \embed\ size $d\!=\!512$, most likely due to the vast increase in parameter count necessitating more training. In the original ViT, multiple encoding blocks were needed before the model could exhibit performance equivalent to their baseline CNN \cite{dosovitskiy2020image}, as verified in our ablation with our ViT. However, for ViTCA we notice an inverse relationship of the effect of Transformer depth, causing a divergence in cell state. It is not clear why this is the case, as we have observed that the LN layers and overflow losses otherwise encourage a contractive $F_\theta$. This is an investigation we leave for future work. Despite the benefits of increasing $h$, we use $h\!=\!4$ for our baseline to optimize runtime performance. Finally, we show that ViTCA does not dramatically suffer when no explicit positioning is used---in contrast to typical Transformer-based models---as cells are still able to localize themselves by relying on their stored hidden information.

\vspace{-.5\baselineskip}
\subsubsection{Cell state analysis}
\label{subsubsec:cell_state_analysis}
\vspace{-.5\baselineskip}

Here we provide an empirically-based qualitative analysis on the effects ViTCA and UNetCA have on cell states through several experiments with our pre-trained models (\Fig{\ref{fig:analysis} (a,b,c)}). We notice that in general, ViTCA indefinitely maintains cell state stability while UNetCA typically induces a divergence past a certain point. An extended analysis is available in Appendix \ref{subsec:extended_analysis}.

% \looseness=-1  % prepend to paragraphs if need to deal with single word consuming a line
\textbf{Damage resilience.}
% Explain damaging scheme. Talk about how it wasn't even trained for this and yet it is extremely robust against cell damage, which is something other CA approaches had to do.
% Damage scheme is even more intense than VNCA's damage scheme. Where they only damaged one spot and not repeatedly damaging multiple spots. Also, ours didn't leave behind an artefact resembling the outline of the damage patch.
% Figure(s) showcasing damage and recovery for MNIST, FashionMNIST, and LandCoverRep.
% Include videos in supplementary.
Shown in \Fig{\ref{fig:analysis}} (a), we damage a random $H/2\!\times\!W/2$ patch of cells with random values $\sim\!\mathcal{U}(-1,1)$ twice in succession. ViTCA is able to maintain cell stability despite not being trained to deal with such noise, while UNetCA induces a divergence. Note both models are simultaneously performing the typical denoising task. We also note that ViTCA's inherent damage resilience is in contrast to recent NCA formulations that required explicit training for it \cite{palm2022variational,mordvintsev2020growing}.

\textbf{Convergence stability.}
% Talk about stability of cells once they reach convergence and how it compares with UNetCA.
% Talk about stability of training and how layernorm layers help. Also mention how even layernorm layers aren't necessarily needed to ensure cell state stability due to overflow losses.
% Figures showing how UNetCA diverges after 800(?) iters and how ViTCA still hasn't after 3k iters for all 4 datasets.
% Include videos in supplementary.
\Fig{\ref{fig:analysis}} (b) shows denoising results after 2784 cell grid updates. ViTCA is able to maintain a stable cell grid state while UNetCA causes cells to diverge.

\textbf{Hidden state visualizations.}
% Include videos and pics in supplementary.
\Fig{\ref{fig:analysis}} (c) shows 2D and 3D PCA dimensionality reductions on the hidden states of converged cell grids for all examples in FashionMNIST~\cite{xiao2017fashion}. The clusters suggest some linear separability in the learned representation, motivating our probing experiments in \Sec{\ref{subsec:probing}}. 

\input{figures/analysis}

% \vspace{-.5\baselineskip}
\subsubsection{Investigating update rule inductive biases}
\label{subsubsec:inductive_bias_investigation}
\vspace{-.5\baselineskip}

Here we investigate the inductive biases inherent in ViTCA and UNetCA by testing their adaptation to various environmental changes (\Fig{\ref{fig:analysis}} (d,e,f,g,h)).

\textbf{Adaptation to varying update rates.}
% Include videos in supplementary.
Despite being trained with a $\sigma\!=\!50\%$ cell update rate, ViTCA is able to adapt to varying rates (\Fig{\ref{fig:analysis}} (d)). Higher rates result in a proportionally faster rate of cell state convergence, and equivalently with lower rates. UNetCA exhibits a similar relationship, although is unstable at $\sigma\!=\!100\%$ (see Appendix \ref{subsec:extended_analysis}). For details comparing training with a synchronous \vs asynchronous cell grid update, see Appendix \ref{subsec:extended_ablation}.

\textbf{Generalization to noise unseen during training.}
% Include videos in supplementary.
ViTCA is capable of denoising configurations of noise it has not been trained on. \Fig{\ref{fig:analysis}} (e; \emph{left-to-right}): $4\!\times\!1$ and $1\!\times\!4$ patches of Gaussian noise at 65\% coverage. In contrast, UNetCA induces a cell state divergence (see Appendix \ref{subsec:extended_analysis}).

\textbf{Adaptation to changing inputs.}
% Include videos in supplementary.
At various moments during cell updates, we re-inject cells with new masked inputs (\Fig{\ref{fig:analysis}} (f)). ViTCA is able to consistently adapt cells to new inputs while UNetCA experiences difficulty past a certain point (\eg at 464 iterations in the figure).

\textbf{Effects of not \vs completely masking input.}
% (not masking) Showcases model able to do autoencoding despite not being trained for it
% (completely masking) Showcases inductive bias of model. CelebA results are interesting since it shows the median face. ViTCA is still able to stabilize while UNetCA diverges.
\Fig{\ref{fig:analysis}} (g; \emph{left}): ViTCA is able to perform autoencoding despite not being trained for it. UNetCA induces a cell grid divergence (see Appendix \ref{subsec:extended_analysis}). \Fig{\ref{fig:analysis}} (g; \emph{right}): Interestingly, when the input is completely masked, ViTCA outputs the median image~\cite{lehtinen2018noise2noise}. UNetCA does not exhibit such behaviour and instead causes cells to diverge (see Appendix \ref{subsec:extended_analysis}). 

\textbf{Spatial interpolation.}
% Reference CPPNs and NeRFs and other coordinate-based neural representations.
% Compare between nerf and vit pe approaches in how they affect spatial interpolation.
% Ruminate on how explicit cell positioning is required to enable this feature, which sort of goes against the self-organizing nature of cells (the position info should be encoded implicitly within each cell's hidden representation). EDIT: actually, no positional encoding is needed at all! It works without it :)
% Figures showing CelebA and FashionMNIST denoising at higher resolutions despite not being trained for it. Scale of noise remains the same but there's more image information than before. (Generalization to noise unseen during training)
% Mention how UNetCA results aren't as good and tend to diverge past a certain point. Don't have results to show because lack of time.
% Include videos in supplementary.
We use ViTCA models trained at $32\!\times\!32$ using various types of positioning to generate $128\!\times\!128$ outputs during inference, assuming an identical cell grid resolution. \Fig{\ref{fig:analysis}} (h; \emph{top-to-bottom of \textcolor{vitcaPurple}{outputs}}): xy-coordinates, no positioning, Fourier features \cite{mildenhall2020nerf}, Fourier features concatenated with xy-coordinates, and a Transformer-based handcrafted positional encoding (baseline) \cite{vaswani2017attention}. Results are ordered from best to worst. The baseline approach is not capable of spatial interpolation due to being a 1D positioning, while, as expected, the 2D encodings make it capable. Surprisingly, removing Fourier features and using only xy-coordinates results in a higher fidelity interpolation. We believe this to be caused by the distracting amount of positional information Fourier features provide to cells, as cells can instead rely on their hidden states to store higher frequency positional information. Finally, with no explicit positioning, ViTCA is still able to perform high-quality interpolation---even exceeding using Fourier features---by taking advantage of its self-organizing nature. As a side note, we point attention to the fact that ViTCA is simultaneously denoising at a scale space it has not been trained on, exemplifying its generalization capabilities.

\vspace{-.5\baselineskip}
\subsection{Investigating hidden representations via linear probes}
\vspace{-.5\baselineskip}
\label{subsec:probing}

% Explain task and datasets used
% Include table comparing linear classification performance on representations from the chosen models, and also compare with linear and non-linear classification on raw pixels.
% Correlation between denoising performance and linear probe performance on certain datasets.
% Relate to PCA visualization where clusters were formed in certain datasets.
\input{tables/linear_probe_results}
Here we examine the learned representations of our models pre-trained for denoising.  We freeze model parameters and learn linear classifiers on each of their learned representations: converged cell hidden states for CA-based models, bottleneck features for U-Net, and LN'd tokens for ViT. This is a common approach used to probe learned representations~\cite{chen2020generative}. Classification results on MNIST, FashionMNIST, and CIFAR10 are shown in \Tab{\ref{tab:linear_probe_results}} and we use the same training setup as for denoising, but without any noise. For comparison, we also provide results using a linear classifier and two 2-layer MLPs of varying complexity, all trained directly on raw pixel values. Correlations between denoising performance in \Tab{\ref{tab:denoising_results}} and classification performance in \Tab{\ref{tab:linear_probe_results}} can be observed. Linear classification accuracy on ViTCA-based features typically exceeds classification accuracy using other model-based features or raw pixel values, even outperforming the MLPs in most cases.

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/analysis.tex <==
\begin{figure}[t]
  \centerline{\includegraphics[scale=1]{analysis.png}}
  \caption{Qualitative results. \textcolor{inGold}{Gold} boxes are inputs, \textcolor{gtGreen}{green} ground truths, \textcolor{vitcaPurple}{purple} ViTCA outputs, and \textcolor{unetcaBlue}{blue} UNetCA outputs. We analyze the effects of ViTCA and UNetCA on cell states in terms of: \textbf{(a)} damage resilience; \textbf{(b)} convergence stabilility, and; \textbf{(c)} hidden state PCA visualizations of converged cell grids for all examples in FashionMNIST~\cite{xiao2017fashion}. We also investigate update rule inductive biases in terms of adapting to: \textbf{(f)} varying inputs \emph{during} cell updates; \textbf{(d)} varying cell update rates; \textbf{(e)} noise configurations unseen during training; \textbf{(g)} unmasked and completely masked inputs, and; \textbf{(h)} spatial interpolation enabled by our various methods of incorporating cell positioning.\vspace{-\baselineskip}}
  \label{fig:analysis}
\end{figure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/attn_head_masking.tex <==
\begin{figure}[t]
  \centerline{\includegraphics[width=\textwidth]{attn_head_masking.png}}
  \caption{Qualitative results showcasing ViTCA's inductive biases in terms of adapting to masking one or several of its self-attention heads. \textcolor{inGold}{Gold} boxes are inputs, \textcolor{gtGreen}{green} ground truths, and \textcolor{vitcaPurple}{purple} ViTCA outputs (after 2784 iterations). For reference, the first column of outputs does not contain any head masking.}
  \label{fig:attn_head_masking}
\end{figure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/fusion_mitosis.tex <==
\ffigbox[0.4\textwidth]{
  \centerline{\includegraphics[width=\FBwidth]{fusion_mitosis.png}}
}{
  \caption{Qualitative results using cell fusion and mitosis as an alternative to gradient checkpointing. \textcolor{inGold}{Gold} boxes are inputs, \textcolor{gtGreen}{green} ground truths, \textcolor{vitcaPurple}{purple} ViTCA outputs, and \textcolor{unetcaBlue}{blue} ViTCA w.\ fusion and mitosis outputs. Outputs are after 64 CA iterations.}
  \label{fig:fusion_mitosis}
}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/overview.tex <==
\begin{figure}[t]
  \centerline{\includegraphics[scale=1]{overview.png}}
  \caption{\textbf{Computational overview}. NCAs use a stateful lattice of \emph{cells}, each storing information along channels, to promote desired behaviour over the course of an evolutionary cycle. Starting from an initial seed, each cell state evolves at discrete time steps according to a homogeneous, learned \emph{update rule} applied either synchronously or asynchronously ($\sigma$). This update depends on the current cell state and that of its \emph{neighbours} (pictured is the \emph{Moore neighbourhood}~\cite{weissteinmoore}). In \textbf{ViTCA}, each cell is represented as a vector where the first $C_iP_HP_W$ channels contain a $P_H \times P_W$ noisy input image patch (\maskedinputsmall), the next $C_oP_HP_W$ channels contain the current output patch (\currentoutput), the following $C_h$ channels contain undefined data hidden from the loss that can be used to encode additional information (\currenthidden), and (optionally) the remaining $C_{\peplain}P_HP_W$ channels contain positional information (\pe). The update rule ($F_\theta$) is a modified ViT \cite{dosovitskiy2020image} whose self-attention mechanism is locally constrained to each cell's neighbourhood (\localize).\vspace{-\baselineskip}}
  \label{fig:overview}
\end{figure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/teaser.tex <==
\begin{figure}[t]
  \centerline{\includegraphics[scale=0.9]{teaser.png}}
  \caption{\textbf{Global self-organization manifested within localized self-attention}. Despite operating in spatially local neighbourhoods about a cell, over time the localized (multi-head) self-attention in ViTCA experiences a \emph{global} self-organization admitted by its NCA nature. This circumvents the quadratic complexity of explicit global self-attention (\wrt input size) with a linear amortization over time (recurrent CA iterations), enabling effective per-pixel dense processing. \emph{Middle}: visualizing local attention maps about each cell as colour-coded ``splats'' blended together in overlapping regions, producing a ``splat map''~\cite{crawfis1993texture}. \emph{Left, right}: ViTCA iterations on a cell grid, updated from a seed state to a converged state, given a noisy input image to denoise. For each head of the cells' local attention maps, there is global agreement on the types of features to attend to (\eg foreground contours, noise, background). Enveloping ViT by the NCA paradigm dramatically improves its output fidelity.\vspace{-\baselineskip}}
  \label{fig:teaser}
\end{figure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/unetca_extended_analysis.tex <==
\begin{figure}[t]
  \centerline{\includegraphics[scale=1]{unetca_extended_analysis.png}}
  \caption{Qualitative results showcasing UNetCA's inductive biases in terms of adapting to: \textbf{(a)} varying cell update rates; \textbf{(b)} noise configurations unseen during training, and; \textbf{(c)} unmasked and completely masked inputs. \textcolor{inGold}{Gold} boxes are inputs, \textcolor{gtGreen}{green} ground truths, and \textcolor{unetcaBlue}{blue} UNetCA outputs.\vspace{-\baselineskip}}
  \label{fig:unetca_extended_analysis}
\end{figure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/figures/vitca_vs_vit.tex <==
\begin{wrapfigure}{r}[0pt]{0.5\textwidth}
  \vspace{-\baselineskip}
  \centerline{\includegraphics[width=\textwidth]{vitca_vs_vit.png}}
  \caption{\textbf{ViT} \vs\ \textbf{ViTCA} for denoising Tiny ImageNet \cite{russakovsky2015imagenet} validation set images with 2$\times$2 pixel masks covering $75\%$ of the image. \emph{Top-to-bottom}: noisy input, ViT, ViTCA, and ground truth.\vspace{-\baselineskip}} 
  \label{fig:vitca_vs_vit}
\end{wrapfigure}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/introduction.tex <==
\section{Introduction}
\vspace{-.5\baselineskip}
\label{sec:introduction}

\input{figures/vitca_vs_vit} Recent developments at the intersection of two foundational ideas---Artificial Neural Networks (ANNs) and Cellular Automata (CA)---have led to new approaches for constructing Neural Cellular Automata (NCA). These advances have integrated ideas such as variational inference \cite{palm2022variational}, U-Nets \cite{zhang2020learning}, and Graph Neural Networks (GNNs) \cite{grattarola2021learning} with promising results on problems ranging from image synthesis \cite{palm2022variational,niklasson2021self-organising,mordvintsev2021mu} to Reinforcement Learning (RL) \cite{najarro2022hypernca,variengien2021towards}. Transformers are another significant development in deep learning \cite{vaswani2017attention}, but, until now, have not been examined under an NCA setting.

Vision Transformers (ViTs) \cite{dosovitskiy2020image} have emerged as a competitive alternative to Convolutional Neural Network (CNN) \cite{lecun1998gradient} architectures for computer vision, such as Residual Networks (ResNets) \cite{he2016deep}. ViTs leverage the self-attention mechanisms of original Transformers \cite{vaswani2017attention}, which have emerged as the dominant approach for sequence modelling in recent years. Our work combines foundational ideas from Transformers and ViTs, leading to a new class of NCAs: \textbf{Vision Transformer Cellular Automata (ViTCA)}. 

An effective and ubiquitous Transformer-based learning technique for Natural Language Processing (NLP) pre-training is the unsupervised task of Masked Language Modelling (MLM), popularized by the BERT language model \cite{devlin-etal-2019-bert}. The success of MLM-based techniques has similarly inspired recent work re-examining the classical formulation of Denoising Autoencoders (DAEs) \cite{vincent2010stacked}, but for ViTs \cite{bao2022beit,dosovitskiy2020image,chen2020generative}, introducing tasks such as Masked Image Encoding \cite{he2021masked} and Masked Feature Prediction \cite{wei2021masked} for image and video modelling, respectively. This simple yet highly-scalable strategy of masked-based unsupervised pre-training has yielded promising transfer learning results on vision-based downstream tasks such as object detection and segmentation, image classification, and action detection, even outperforming supervised pre-training~\cite{he2021masked,wei2021masked}. We examine training methodologies for ViTCA within a DAE setting and perform extensive controlled experiments benchmarking these formulations against modern state of the art architectures, with favourable outcomes, \eg \Fig{\ref{fig:vitca_vs_vit}}.

\input{figures/teaser}

Our contributions are as follows: \textit{first}---to the best of our knowledge---our work is the first to extend NCA methodologies with key Transformer mechanisms, \ie self-attention and positional encoding (and embedding), with the beneficial side-effect of circumventing the quadratic complexity of self-attention; \textit{second}, our ViTCA formulation allows for lower model complexity (by limiting ViT depth) while retaining expressivity through CA iterations on a controlled state---all with the same encoder weights. This yields a demonstrably more parameter-efficient \cite{mordvintsev2021mu} ViT-based model. Importantly, ViTCA mitigates the problems associated with the explicit tuning of ViT depth originally needed to improve performance (\ie we use a depth of 1). With ViTCA, we simply iterate until cell state convergence. Since ViT (and by extension, ViTCA) employs Layer Normalization (LN) \cite{ba2016layer} at each stage of its processing, it is a fairly contractive model capable of fixed-point convergence guarantees~\cite{bai2019deep}.

In relation to our first contribution, ViTCA respects CA requirements, most importantly that computations remain localized about a cell and its neighbourhood. As such, we modify the global self-attention mechanisms of a ViT to respect this locality requirement (\Fig{\ref{fig:teaser}}). Localized self-attention is not a new idea \cite{chen2022regionvit,liu2021swin,chu2021twins,zhang2021multi}; however, because cells contain state information that depends on its previous state, over CA iterations the effective receptive field of ViTCA's localized self-attention grows increasingly larger until eventually incorporating information implicitly across all cells. Thus, admitting global propagation of information from spatially localized self-attention. Moreover, due to the self-organizing nature of NCAs, self-organization also manifests itself within the localized self-attention, resulting in a globally agreed-upon arrangement of local self-attention. Thus, circumventing the quadratic complexity of explicit global self-attention (\wrt the input size) through a linear amortization over time, and increasing the feasibility of per-pixel dense processing (as we demonstrate). This globally consistent and complex behaviour, which arises from strictly local interactions, is a unique feature of NCAs and confers performance benefits which we observe both qualitatively and quantitatively when comparing ViT and ViTCA for denoising autoencoding. 

\input{figures/overview}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/related_work.tex <==
\vspace{-.5\baselineskip}
\section{Background and related work}
\vspace{-.5\baselineskip}
\label{sec:related_work}

\paragraph{Neural Cellular Automata.}

Cellular Automata are algorithmic processes motivated by the biological behaviours of cellular growth and, as such, are capable of producing complex emergent (global) dynamics from the iterative application of comparatively simple (localized) rules~\cite{von1966theory}. \emph{Neural} Cellular Automata present a more general CA formulation, where the evolving cell states are represented as (typically low-dimensional) vectors and the update rule dictating their evolution is a differentiable function whose parameters are learned through backpropagation from a loss, rather than a handcrafted set of rules~\cite{mordvintsev2020growing,gilpin2019cellular,wulff1992learning}.
Neural net-based formulations of CAs in the NeurIPS community can be traced back to the early work of \cite{wulff1992learning}, where only small and simple models were examined. Recent formulations of NCAs have shown that when leveraging the power of deep learning techniques enabled by advances in hardware capabilities---namely highly-parallelizable differentiable operations implemented on GPUs---NCAs can be tuned to learn surprisingly complex desired behaviour, such as semantic segmentation \cite{sandler2020image}; common RL tasks such as cart-pole balancing \cite{variengien2021towards}, 3D locomotion \cite{najarro2022hypernca}, and Atari game playing \cite{najarro2022hypernca}; and image synthesis~\cite{palm2022variational,niklasson2021self-organising,mordvintsev2021mu}. Although these recent formulations rely on familiar compositions of convolutions and non-linear functions, it is important to highlight that NCAs are fundamentally not equivalent to ``very-deep'' CNNs (\vs~\cite{gilpin2019cellular}), or any other feedforward architecture (\eg ResNets \cite{he2016deep}), particularly, in the same way that a Recurrent Neural Network (RNN) is not equivalent: CNNs and other feedforward architectures induce a directed \textit{acyclic} computation graph (\ie a finite impulse response), whereas NCAs (and RNNs) induce a directed \textit{cyclic} computation graph (\ie an infinite impulse response), where stateful data can additionally be manipulated using (learned) feedback loops and/or time-delayed controls. As such, NCAs can be viewed as a type of RNN, and both (N)CAs and RNNs are known to be Turing complete~\cite{christen2021automatic,cook2004universality,siegelmann1995computational,wulff1992learning}.\footnote{In the case of (N)CAs, a Turing complete example is the \emph{Rule 110} elementary CA \cite{christen2021automatic,cook2004universality}}
% specifically, RNNs generally learn compositions of the form $f_0 \circ f_1 \circ \ldots \circ f_n$, whereas NCAs learn the same form of compositions as RNNs \textit{with weight sharing}, namely $f \circ  \ldots \circ f$. We will show that extending NCAs with Transformers results in the ability to learn compact, stable, and complex recurrent processes.
%
% Check this response from the authors https://openreview.net/forum?id=7fFO4cMBx_9&noteId=1dYLpi1TzpB
% NCAs are a class of CNNs but that's not the point <-- mattie: incorrect, they are not a class of CNNs, as I incorrectly stated during our meeting
%
% See https://mila-umontreal.slack.com/archives/C02166S2W1W/p1651756000775349. In short, you can say that an NCA is a neural network that uses convolutions, but differs from a convolutional network in that you _can not_ unroll it and replace it with a feedforward network. An NCA is a directed cyclic graph while a convolutional network is a directed _acyclic_ graph. In other words, an NCA is part of a class of networks with infinite impulse response whereas convolutional networks are a class of networks with finite impulse response. Both finite and infinite impulse response networks (see below for definition) can have additional stored states that can be controlled by the network, the difference being that an infinite impulse response network incorporates feedback loops and/or time delays to control the stored state in a time-indefinite fashion. This is traditionally called a Recurrent Neural Network and any off-the-shelf RNN can replace ViTCA. Our contribution is that instead of using common instantiations of RNNs, like an LSTM or a GRU or even basic convolutions with non-linearities (I'm taking care not to say conv net here, and networks such as LSTMConv do not count as they are hybrids), we use a Transformer. Not many papers have used Transformers as RNNs (see Related Works google doc https://docs.google.com/document/d/1jGI-js94HgFx2KgHDKzPyywCmsxToQYbgjsdy_tDUUk/edit#).
%
% Something to note of infinite impulse networks is that the controlled state can exhibit certain patterns of behaviour after an amount of time. 1. The state can converge to a fixed-point (either a trivial or non-trivial solution, depending on the PDE); 2. The state can oscillate about a fixed-point (because step size is too big); 3. The state can jump and oscillate about multiple fixed-points but remain bounded within a basin of attraction (also called radius/region of convergence); 4. The state can diverge due to multiple reasons: a) the network can not find a fixed-point attractor and thus diverges the state from its initial state (either because of poor initialization or because there is no solution), b) the state nearly reaches stable convergence but due to overly ambitious steps towards the fixed point, it soon diverges outside of any region of convergence, c) adversarial attacks and perturbations knock the state outside of any region of convergence. These 4 patterns of behaviour are encapsulated within an analogous NCA classification system defined by Wolfram:
% Class 1: Nearly all initial patterns evolve quickly into a stable, homogeneous state. Any randomness in the initial pattern disappears.
% Class 2: Nearly all initial patterns evolve quickly into stable or oscillating structures. Some of the randomness in the initial pattern may filter out, but some remains. Local changes to the initial pattern tend to remain local.
% Class 3: Nearly all initial patterns evolve in a pseudo-random or chaotic manner. Any stable structures that appear are quickly destroyed by the surrounding noise. Local changes to the initial pattern tend to spread indefinitely.
% Class 4: Nearly all initial patterns evolve into structures that interact in complex and interesting ways, with the formation of local structures that are able to survive for long periods of time.[33] Class 2 type stable or oscillating structures may be the eventual outcome, but the number of steps required to reach this state may be very large, even when the initial pattern is relatively simple. Local changes to the initial pattern may spread indefinitely. Wolfram has conjectured that many class 4 cellular automata, if not all, are capable of universal computation. This has been proven for Rule 110 and Conway's Game of Life.
%
% Comparisons can be drawn between numerical analysis and signal processing, namely Lipschitz continuity and Bounded-Input, Bounded-Output (BIBO) stability and how both of these definitions can be used to describe cell state behaviour (and required behaviour if an implicit method is used to solve the cell state, as described below, since it requires the update rule to be contractive/Lipschitz continuous)
%
% See https://mila-umontreal.slack.com/archives/C02166S2W1W/p1651756103476509. Infinite impulse response (IIR) is a property applying to many linear time-invariant systems that are distinguished by having an impulse response h(t) which does not become exactly zero past a certain point, but continues indefinitely. This is in contrast to a finite impulse response (FIR) system in which the impulse response  does become exactly zero at times t>T for some finite T, thus being of finite duration. Common examples of linear time-invariant systems are most electronic and digital filters. Systems with this property are known as IIR systems or IIR filters.
%
% Take a look at https://distill.pub/selforg/2021/textures/ specifically the "PDEs" section. The NCA update rule describes a partial differential equation modeling a reaction-diffusion dynamical system (not unlike the Gray-Scott model of reaction-diffusion) that is solved through discretized steps. Since the evaluation of cell states is time-discretized into fixed-size steps, we can say it is equivalent to explicit Euler integration of an N-order PDE (I know Euler's method is typically used to solve 1st-order ODEs, but you can represent any N-order ODE as a system of 1st-order ODEs and solve with Euler's method, so I think it's okay to say the NCA update rule is an explicit Euler integrator). Technically, you can replace the ViTCA-based NCA update rule with any other PDE solver, like some other RK-based explicit method (like how the Neural ODE paper replaced layers in a resnet with ODE solvers each performing a linear multistep method like implicit Adams, or replacing layers with their RK-Net https://proceedings.neurips.cc/paper/2018/file/69386f6bb1dfed68692a24c8686939b9-Paper.pdf). 
%
% We can say that for future work we can investigate explicit methods of integration during the forward pass (described above) and implicit methods of integration during the forward pass (e.g., backward Euler + fixed-point iterations via Newton's/Quasi-Newton method to solve for the fixed-point/root G(y(x, t), y(x, t+delta)) = 0 where y is the update rule that outputs the next cell state and x is the injected input). We can also say that for future work this can be applied for the backward pass as well (i.e., implicit diff, DEQ). Both have their merits: first allows for a more accurate (and thus, faster, and potentially eliminating oscillating states) convergence and second removes memory limitations during backward pass (could also use the "phantom gradient" method to get nearly-computation-free gradients, see https://arxiv.org/pdf/2204.08442.pdf and https://arxiv.org/abs/2111.05177).

\paragraph{Vision Transformers.}
Vision Transformers \cite{dosovitskiy2020image} are an adaptation of Transformers \cite{vaswani2017attention} to vision-based tasks like image classification. In contrast to networks built from convolutional layers, ViTs rely on \emph{self-attention} mechanisms operating on tokenized inputs. Specifically, input images are divided into non-overlapping patches, then fed to a Transformer after undergoing a linear patch projection with an embedding matrix. While ViTs provide competitive image classification performance, the quadratic computational scaling of global self-attention limits their applicability in high-dimensional domains, \eg per-pixel dense processing. Recent developments have attempted to alleviate such efficiency limitations \cite{ali2021xcit,hudson2021generative,arnab2021vivit,fan2021multiscale}, one notable example being Perceiver IO \cite{jaegle2021perceiver,yifan2021input} with its use of cross-attention. We refer interested readers to a comprehensive survey on ViTs~\cite{khan2021transformers}.

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/ablation_results.tex <==
\begin{wraptable}[44]{r}{0.515\textwidth}
  \caption{Quantitative ablation for denoising autoencoding with ViTCA (unless otherwise stated via prefix) on CelebA \cite{liu2015faceattributes}. Boldface and underlining denote best and second best results. Italicized items denote baseline configuration settings. \ts\textdagger Trained with gradient checkpointing \cite{chen2016training}, which slightly alters round-off error during backpropagation, resulting in slight variations of results compared to training without checkpointing. See Appendix \ref{subsec:extended_ablation}.}
  \label{tab:ablation_results}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{6}{l}@{}}
        & & {\psnrlabel} & {\ssimlabel} & {\lpipslabel} & {\paramslabel} \\
        \toprule
        \multirow{7}{*}{\rot{\textbf{Hidden dim}}}
        & 8 & 25.61 & 0.898 & 0.086 & 86.3K \\
        & 16 & 26.11 & 0.909 & 0.070 & 88.4K \\
        & \textit{32} & 26.53 & 0.913 & \underline{0.066} & 92.5K \\
        & 64 & 26.53 & 0.913 & \underline{0.066} & 100.7K \\
        & 128 & 26.51 & 0.912 & \underline{0.066} & 117.2K \\
        & 256 & \underline{26.77} & \underline{0.915} & \textbf{0.063} & 150.1K \\
        & 512 & \textbf{26.78} & \textbf{0.916} & \textbf{0.063} & 215.9K \\
        \midrule[\heavyrulewidth]
        \multirow{7}{*}{\rot{\textbf{Embed dim}}}
        & 8\ts\textdagger & 21.67 & 0.814 & 0.258 & 2.0K \\
        & 16\ts\textdagger & 23.22 & 0.853 & 0.183 & 4.5K \\
        & 32\ts\textdagger & 24.94 & 0.875 & 0.110 & 10.9K \\
        & 64\ts\textdagger & 25.69 & 0.898 & 0.084 & 29.9K \\
        & \textit{128}\ts\textdagger & \underline{26.05} & \underline{0.904} & \underline{0.075} & 92.5K \\
        & 256\ts\textdagger & \textbf{26.36} & \textbf{0.911} & \textbf{0.067} & 316.0K \\
        & 512\ts\textdagger & 19.93 & 0.768 & 0.274 & 1.2M \\
        \midrule[\heavyrulewidth]
        \multirow{6}{*}{\rot{\textbf{Heads}}}
        & 1 & 25.01 & 0.890 & 0.096 & 76.0K \\
        & \textit{4} & 26.53 & 0.913 & 0.066 & 92.5K \\
        & 8 & 26.77 & 0.916 & 0.062 & 92.5K \\
        & 16 & 26.78 & 0.917 & 0.062 & 92.5K \\
        & 32 & \textbf{27.01} & \textbf{0.920} & \textbf{0.060} & 92.5K \\
        & 64 & \underline{26.94} & \underline{0.919} & \underline{0.061} & 92.5K \\
        \midrule[\heavyrulewidth]
        \multirow{6}{*}{\rot{\textbf{Depth}}}
        & \emph{ViTCA--1} & \textbf{26.53} & \textbf{0.913} & \textbf{0.066} & 92.5K \\
        & ViTCA--2\ts\textdagger & \underline{10.82} & \underline{0.225} & \underline{0.771} & 175.3K \\
        & ViTCA--3\ts\textdagger & 9.70 & 0.165 & 0.793 & 258.0K \\
        \cmidrule(l){2-6}
        & \emph{ViT--1} & 19.70 & 0.779 & 0.237 & 83.9K \\
        & ViT--2\ts\textdagger & \underline{25.20} & \underline{0.900} & \underline{0.074} & 166.7K \\
        & ViT--3\ts\textdagger & \textbf{26.10} & \textbf{0.914} & \textbf{0.065} & 249.4K \\
        \midrule[\heavyrulewidth]
        \multirow{6}{*}{\rot{\textbf{PE type}}}
        & sincos5 & \underline{26.92} & \underline{0.917} & \underline{0.062} & 95.1K \\
        & sincos5xy & \textbf{27.00} & \textbf{0.919} & \textbf{0.059} & 95.3K \\
        & xy & 26.45 & 0.894 & 0.077 & 92.8K \\
        & \textit{handcrafted} & 26.53 & 0.913 & 0.066 & 92.5K \\
        & learned & 26.16 & 0.910 & 0.071 & 223.6K \\
        & none & 26.28 & 0.890 & 0.081 & 92.5K \\
        \bottomrule
        &&&&&\\ 
    \end{tabular}
    \vspace{-\baselineskip}
\end{wraptable}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/attn_size_ablation_results.tex <==
\begin{table}[t!]
  \caption{Quantitative ablation on attention neighbourhood size $N_H\times N_W$ for denoising autoencoding with ViTCA on FashionMNIST. Boldface and underlining denote best and second best results. Italicized items denote baseline configuration settings.}
  \label{tab:attn_size_ablation_results}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{4}{l}@{}}
        & \psnrlabel & \ssimlabel & \lpipslabel \\
        \toprule
        \textit{3$\times$3} & \textbf{23.25} & \textbf{0.827} & \textbf{0.145} \\
        5$\times$5 & \underline{22.34} & \underline{0.817} & \textbf{0.145} \\
        7$\times$7 & 21.65 & 0.792 & \underline{0.168} \\
        \bottomrule
    \end{tabular}
\end{table}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/denoising_results.tex <==
\begin{table}[t!]
  \caption{Comparing denoising autoencoding results between baselines and ViTCA variants. ViTCA variants include: 32 (32 heads), 16 (16 heads), i (inverted bottleneck), xy (xy-coordinate positional encoding). Boldface and underlined values denote the best and second best results. Metrics include Peak Signal-to-Noise Ratio (PSNR; dB), Structural Similarity Index Measure (SSIM; values in $[0,1]$) \cite{wang2004image}, Learned Perceptual Image Patch Similarity (LPIPS; values in $[0, 1]$) \cite{zhang2018unreasonable}.\vspace{-\baselineskip}}
  \label{tab:denoising_results}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{14}{l}@{}}
        & & \multicolumn{4}{c}{\textbf{LandCoverRep}} & \multicolumn{4}{c}{\textbf{CelebA}} & \multicolumn{4}{c}{\textbf{MNIST}} \\
        \cmidrule[\heavyrulewidth](lr){3-6} \cmidrule[\heavyrulewidth](lr){7-10}
        \cmidrule[\heavyrulewidth](lr){11-14}
        \addlinespace[-\aboverulesep]
        & & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\paramslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\paramslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\paramslabel} \\
        \toprule
        \multirow{4}{*}{\rot{\textbf{Baselines}}}
        & U-Net & 33.94 & 0.934 & \textbf{0.099} & 106.6K & 26.23 & 0.906 & 0.075 & 106.6K & 23.43 & 0.897 & 0.049 & 104.5K \\
        & ViT & 30.64 & 0.893 & 0.135 & 83.9K & 19.70 & 0.779 & 0.237 & 83.9K & 16.02 & 0.631 & 0.254 & 83.4K \\
        & UNetCA & 33.94 & \underline{0.935} & \underline{0.102} & 54.0K & 25.66 & 0.882 & 0.091 & 54.0K & 25.61 & 0.929 & 0.034 & 52.0K \\
        & ViTCA & 33.80 & 0.932 & \underline{0.102} & 92.5K & 26.53 & \underline{0.913} & \underline{0.066} & 92.5K & \underline{27.01} & 0.940 & \underline{0.028} & 91.7K \\
        \cdashrule{1-14}
        \multirow{6}{*}{\rot{\textbf{Variants}}}
        & ViTCA-32 & \underline{34.00} & \underline{0.935} & 0.103 & 92.5K & \textbf{27.01} & \textbf{0.920} & \textbf{0.060} & 92.5K & \textbf{27.68} & \textbf{0.946} & \textbf{0.026} & 91.7K \\
        & ViTCA-32xy & \textbf{34.06} & \textbf{0.936} & 0.106 & 92.8K & \underline{26.75} & 0.898 & 0.072 & 92.8K & 26.97 & \underline{0.942} & \underline{0.028} & 92.0K \\
        & ViTCA-i & 33.49 & 0.929 & 0.108 & 54.7K & 26.10 & 0.904 & 0.074 & 54.7K & 26.03 & 0.930 & 0.033 & 54.3K \\
        & ViTCA-i16 & 33.74 & 0.932 & 0.106 & 54.7K & 26.61 & 0.912 & \underline{0.066} & 54.7K & 26.42 & 0.935 & 0.031 & 54.3K \\
        & ViTCA-ixy & 33.75 & 0.933 & 0.107 & 54.8K & 26.51 & 0.894 & 0.076 & 54.8K & 25.95 & 0.933 & 0.033 & 54.4K \\
        & ViTCA-i16xy & 33.93 & \underline{0.935} & 0.108 & 54.8K & 26.68 & 0.898 & 0.074 & 54.8K & 26.28 & 0.936 & 0.031 & 54.4K \\
        \bottomrule
    \end{tabular}
    \begin{tabular}{@{}*{14}{l}@{}}
        \addlinespace[\aboverulesep]
        & & \multicolumn{4}{c}{\textbf{FashionMNIST}} & \multicolumn{4}{c}{\textbf{CIFAR10}} & \multicolumn{4}{c}{\textbf{Tiny ImageNet}} \\
        \addlinespace[-\aboverulesep]
        \cmidrule[\heavyrulewidth](lr){3-6} \cmidrule[\heavyrulewidth](lr){7-10}
        \cmidrule[\heavyrulewidth](lr){11-14}
        \addlinespace[-1pt]
        \toprule
        \multirow{4}{*}{\rot{\textbf{Baselines}}}
        & U-Net & 24.19 & 0.852 & 0.126 & 104.5K & 25.62 & 0.855 & 0.131 & 106.6K & 21.93 & 0.775 & 0.203 & 106.6K \\
        & ViT & 16.28 & 0.519 & 0.397 & 83.4K & 20.99 & 0.744 & 0.237 & 83.9K & 17.80 & 0.598 & 0.355 & 83.9K \\
        & UNetCA & 23.67 & 0.854 & 0.123 & 52.0K & 25.49 & 0.851 & 0.129 & 54.0K & 21.78 & 0.773 & 0.204 & 54.0K \\
        & ViTCA & 23.80 & 0.855 & 0.117 & 91.7K & 25.61 & 0.856 & 0.127 & 92.5K & 21.58 & 0.772 & 0.215 & 92.5K \\
        \cdashrule{1-14}
        \multirow{6}{*}{\rot{\textbf{Variants}}}
        & ViTCA-32 & \textbf{24.91} & \textbf{0.874} & \textbf{0.098} & 91.7K & \underline{26.05} & \underline{0.864} & \underline{0.122} & 92.5K & 21.94 & 0.781 & 0.202 & 92.5K \\
        & ViTCA-32xy & \underline{24.55} & \underline{0.869} & \underline{0.102} & 92.0K & \textbf{26.14} & \textbf{0.866} & \textbf{0.120} & 92.8K & \textbf{22.03} & \textbf{0.783} & \textbf{0.199} & 92.8K \\
        & ViTCA-i & 22.84 & 0.827 & 0.139 & 54.3K & 25.42 & 0.853 & 0.132 & 54.7K & 21.75 & 0.776 & 0.211 & 54.7K \\
        & ViTCA-i16 & 23.32 & 0.839 & 0.127 & 54.3K & 25.65 & 0.856 & 0.128 & 54.7K & 21.72 & 0.774 & 0.213 & 54.7K \\
        & ViTCA-ixy & 23.54 & 0.848 & 0.123 & 54.4K & 25.85 & 0.861 & 0.125 & 54.8K & 21.95 & \underline{0.782} & \underline{0.201} & 54.8K \\
        & ViTCA-i16xy & 23.59 & 0.848 & 0.121 & 54.4K & 25.98 & 0.863 & 0.123 & 54.8K & 21.99 & \underline{0.782} & \underline{0.201} & 54.8K \\
        \bottomrule
    \end{tabular}
\end{table}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/gradient_checkpointing_ablation_results.tex <==
\begin{table}[t!]
  \caption{Quantitative ablation comparing test results of ViTCA trained with gradient checkpointing disabled \vs\ enabled. Boldface denotes best results. Italicized items denote baseline configuration settings.\vspace{-0.5\baselineskip}}
  \label{tab:gradient_checkpointing_ablation_results}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{13}{l}@{}}
        & \multicolumn{3}{c}{\textbf{LandCoverRep}} & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{c}{\textbf{CelebA}} & \multicolumn{3}{c}{\textbf{FashionMNIST}} \\
        \cmidrule[\heavyrulewidth](lr){2-4} \cmidrule[\heavyrulewidth](lr){5-7} \cmidrule[\heavyrulewidth](lr){8-10} \cmidrule[\heavyrulewidth](lr){11-13}
        \addlinespace[-\aboverulesep]
        & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} \\
        \toprule
        \textit{disabled} & \textbf{33.80} & 0.932 & 0.102 & \textbf{27.01} & \textbf{0.940} & \textbf{0.028} & \textbf{26.53} & \textbf{0.913} & \textbf{0.066} & 23.80 & 0.855 & 0.117 \\
        enabled & 33.76 & 0.932 & 0.102 & 26.77 & 0.938 & 0.029 & 26.05 & 0.904 & 0.075 & \textbf{23.89} & 0.855 & 0.117 \\
        \bottomrule
    \end{tabular}
\end{table}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/linear_probe_results.tex <==
\begin{table}[t!]
  \caption{Linear probe \cite{chen2020generative} test accuracies (\%) of baseline and variant models. Model variants are labelled as in \Tab{\ref{tab:denoising_results}}. All baselines and variants were pre-trained for denoising autoencoding and kept fixed during probing. A linear classifier and 2-layer Multilayer Perceptrons (MLP) were trained on raw image inputs. Parameter counts exclude fixed parameters. Boldface and underlined values denote the best and second best results, respectively. Interestingly, CA-based models trained for denoising autoencoding on increasingly challenging datasets produce an increasingly more useful self-supervised representation for image classification compared to non-CA-based models. \vspace{-\baselineskip}}
  \label{tab:linear_probe_results}
  \centering
  \small
    \begin{tabular}{@{}*{8}{l}@{}}
        & & \multicolumn{2}{c}{\textbf{MNIST}} & \multicolumn{2}{c}{\textbf{FashionMNIST}} & \multicolumn{2}{c}{\textbf{CIFAR10}} \\
        \cmidrule[\heavyrulewidth](lr){3-4} \cmidrule[\heavyrulewidth](lr){5-6}
        \cmidrule[\heavyrulewidth](lr){7-8}
        \addlinespace[-\aboverulesep]
        & & \acclabel & \paramslabel & \acclabel & \paramslabel & \acclabel & \paramslabel \\
        \toprule
        \multirow{4}{*}{\rot{\textbf{Baselines}}}
        & U-Net & 96.3 & 15.4K & 86.2 & 15.4K & 52.3 & 15.4K \\
        & ViT & 92.1 & 1.3M & 83.4 & 1.3M & 34.5 & 1.3M \\
        & UNetCA & 96.3 & 327.7K & 89.5 & 327.7K & \textbf{55.1} & 327.7K \\
        & ViTCA & 96.7 & 327.7K & 89.7 & 327.7K & 50.2 & 327.7K \\
        \cdashrule{1-8}
        \multirow{6}{*}{\rot{\textbf{Variants}}}
        & ViTCA-32 & 96.3 & 327.7K & \underline{89.8} & 327.7K & \textbf{55.1} & 327.7K \\
        & ViTCA-32xy & 96.3 & 327.7K & 89.5 & 327.7K & \underline{53.6} & 327.7K \\
        & ViTCA-i & 95.8 & 327.7K & 89.6 & 327.7K & 49.4 & 327.7K \\
        & ViTCA-i16 & 95.7 & 327.7K & \textbf{90.1} & 327.7K & 50.7 & 327.7K \\
        & ViTCA-ixy & 96.2 & 327.7K & 89.6 & 327.7K & 50.2 & 327.7K  \\
        & ViTCA-i16xy & 96.5 & 327.7K & 89.6 & 327.7K & 52.7 & 327.7K \\
        \cdashrule{1-8}
        & Linear classifier & 93.0 & 10.3K & 84.7 & 10.3K & 39.0 & 30.7K \\
        & 2-layer MLP, 100 hidden units & \underline{98.2} & 103.5K & 89.4 & 103.5K & 46.0 & 308.3K \\
        & 2-layer MLP, 1000 hidden units & \textbf{98.5} & 1.0M & 89.6 & 1.0M & 49.7 & 3.1M \\
        \bottomrule
    \end{tabular}
\end{table}


==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/other_ablation_results.tex <==
\capbtabbox[0.56\textwidth]{
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{6}{l}@{}}
        & & \psnrlabel & \ssimlabel & \lpipslabel & \paramslabel \\
        \toprule
        \multirow{7}{*}{\textbf{Pool size}}
        & 128 & 26.51 & \underline{0.914} & \underline{0.065} & 92.5K \\
        & 256 & 26.40 & 0.912 & 0.067 & 92.5K \\
        & 512 & \textbf{26.61} & \textbf{0.915} & \textbf{0.064} & 92.5K \\
        & \textit{1024} & 26.53 & 0.913 & 0.066 & 92.5K \\
        & 2048 & \underline{26.54} & \textbf{0.915} & \textbf{0.064} & 92.5K\\
        & 4096 & 26.48 & 0.912 & 0.066 & 92.5K \\
        & 8192 & 26.30 & 0.910 & 0.069 & 92.5K \\
        \midrule[\heavyrulewidth]
        \multirow{2}{*}{\textbf{Cell init.}}
        & \textit{constant} & \textbf{26.53} & \textbf{0.913} & \textbf{0.066} & 92.5K \\
        & random & \underline{25.90} & \underline{0.905} & \underline{0.074} & 92.5K \\
        \midrule[\heavyrulewidth]
        \multirow{5}{*}{\textbf{Patch size}}
        & \textit{1$\times$1} & \textbf{26.53} & \textbf{0.913} & \textbf{0.066} & 92.5K \\
        & 2$\times$2 & \underline{25.85} & \underline{0.906} & \underline{0.076} & 96.0K \\
        & 4$\times$4 & 24.54 & 0.882 & 0.113 & 109.8K \\
        & 8$\times$8 & 21.62 & 0.803 & 0.212 & 165.3K \\
        & 16$\times$16 & 18.71 & 0.687 & 0.279 & 387.0K \\
        \bottomrule
    \end{tabular}
}{
  \caption{Quantitative ablation on pool size $N_\mathcal{P}$, cell initialization method, and patch size $P_H\times P_W$ for denoising autoencoding with ViTCA on CelebA. Boldface and underlining denote best and second best results. Italicized items denote baseline configuration settings.}
  \label{tab:other_ablation_results}
}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/runtime_profiling_results.tex <==
\begin{wraptable}[15]{r}{0.515\textwidth}
  \caption{Profiling results showcasing ViTCA's runtime performance (forward and backward in milliseconds) and memory usage (in GB) while training on a minibatch of random $32 \times 3 \times H \times W$ images with gradient checkpointing disabled \vs\ enabled. We use $T\!=\!32$ ViTCA iterations and 16 checkpoint segments. Boldface denotes best results. Italicized items denote baseline configuration settings.\vspace{-0.5\baselineskip}}
  \label{tab:runtime_profiling_results} 
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{13}{l}@{}}
        & \diag{\fwdlabel} & \diag{\bwdlabel} & \diag{\memlabel} \\
        \toprule
        \textit{disabled} & \textbf{229ms} & \textbf{355ms} & 17.0GB \\
        enabled & 232ms & 576ms & \textbf{2.5GB} \\
        \bottomrule
    \end{tabular}
\end{wraptable}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/tables/update_rate_ablation_results.tex <==
\begin{table}[t!]
  \caption{Quantitative ablation comparing test results with ViTCA trained using asynchronous ($\sigma\!=\!50\%$) \vs\ synchronous ($\sigma\!=\!100\%$) cell updates for denoising autoencoding. During testing, cells are updated at the rate they were trained in. Boldface denotes best results. Italicized items denote baseline configuration settings.\vspace{-0.5\baselineskip}}
  \label{tab:update_rate_ablation_results}
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}*{13}{l}@{}}
        & \multicolumn{3}{c}{\textbf{LandCoverRep}} & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{c}{\textbf{CelebA}} & \multicolumn{3}{c}{\textbf{FashionMNIST}} \\
        \cmidrule[\heavyrulewidth](lr){2-4} \cmidrule[\heavyrulewidth](lr){5-7} \cmidrule[\heavyrulewidth](lr){8-10} \cmidrule[\heavyrulewidth](lr){11-13}
        \addlinespace[-\aboverulesep]
        & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} & \diag{\psnrlabel} & \diag{\ssimlabel} & \diag{\lpipslabel} \\
        \toprule
        \textit{asynchronous} & \textbf{33.80} & \textbf{0.932} & \textbf{0.102} & \textbf{27.01} & \textbf{0.940} & \textbf{0.028} & \textbf{26.53} & \textbf{0.913} & \textbf{0.066} & \textbf{23.80} & \textbf{0.855} & \textbf{0.117} \\
        synchronous & 33.68 & 0.931 & 0.104 & 26.00 & 0.927 & 0.034 & 23.76 & 0.870 & 0.105 & 23.12 & 0.832 & 0.132 \\
        \bottomrule
    \end{tabular}
\end{table}

==> Attention-based Neural Cellular Automata (NeurIPS '22) arXiv/vitca.tex <==
\vspace{-.5\baselineskip}
\section{Vision Transformer Cellular Automata (ViTCA)}
\vspace{-.5\baselineskip}
\label{sec:vitca}

Building upon NCAs and ViTs, we propose a new class of \emph{attention-based} NCAs formed using a spatially localized---yet globally organized---self-attention scheme. We detail an instance of this class, ViTCA, by first reviewing its backbone ViT architecture before describing the ``pool sampling''-based training process for the ViTCA update rule (see overview in \Fig{\ref{fig:overview}}).

\paragraph{Input tokenization.}

ViT starts by dividing a $C_i\!\times\!H\!\times\!W$ input image \gt\ into $N$ non-overlapping $P_H\!\times\!P_W$ patches ($16\!\times\!16$ in the original work~\cite{dosovitskiy2020image}), followed by a linear projection of the flattened image patches with an embedding matrix $\mathbf{E} \in \mathbb{R}^{L \times d}$ (\Fig{\ref{fig:overview}} \embed), where $L\!=\!C_iP_HP_W$, to produce initial tokens \pretokens\ $\!\in\!\mathbb{R}^{N \times d}$. Next, a handcrafted positional encoding \cite{vaswani2017attention} or learned positional embedding \pe\ $\in\!\mathbb{R}^{N \times d}$ \cite{dosovitskiy2020image} is added to tokens to encode positional information and break permutation invariance. Finally, a learnable class token is appended to the token sequence, resulting with \tokens\ $\!\in\!\mathbb{R}^{(N+1) \times d}$. For the purposes of our task, we omit this token in all ViT-based models. In ViTCA, the input to the embedding is a flattened cell grid \cells\ $\!\in\!\mathbb{R}^{N \times L}$ where $L\!=\!C_PP_HP_W+C_h$, $C_P\!=\!C_i+C_o+C_{\peplain}$,\, $C_h$ is the cell hidden size,\, $C_o$ is the number of output image channels (one or three for grayscale or RGB), and $C_{\peplain}$ is the positional encoding size when positional encoding is (optionally) concatenated to each cell rather than added to the tokens \cite{mildenhall2020nerf}.

\paragraph{Multi-head self-attention (MHSA).}

Given a sequence of tokens \tokens, self-attention estimates the relevance of one token to all others (\eg which image patches are likely to appear together in an image) and aggregates this global information to update each token. This encodes each token in terms of global contextual information, and does so using three learned weight matrices: $\mathbf{W}_Q\!\in\!\mathbb{R}^{d \times d}$, $\mathbf{W}_K\!\in\!\mathbb{R}^{d \times d}$, and $\mathbf{W}_V\!\in\!\mathbb{R}^{d \times d}$. \tokens\ is projected onto these weight matrices to obtain Queries $\mathbf{Q}\!=\!$ \tokens$\mathbf{W}_Q$, Keys $\mathbf{K}\!=\!$ \tokens$\mathbf{W}_K$, and Values $\mathbf{V}\!=\!$ \tokens$\mathbf{W}_V$. The self-attention layer output $\sa\!\in\!\mathbb{R}^{N \times d}$ is:

\input{equations/sa}

\emph{Multi-head} self-attention employs many sets of weight matrices, $\{\mathbf{W}_{Q_i},$ $\mathbf{W}_{K_i},$ $\mathbf{W}_{V_i}\!\in\!\mathbb{R}^{d \times (d/h)}\!\mid$  $i\!=\!0,...,(h-1)\}$. The outputs of $h$ self-attention \emph{heads} are concatenated into $(\sa_0,$ $...,$ $\sa_{h-1})\!\in\!\mathbb{R}^{N \times d}$ and projected onto a weight matrix $\mathbf{W}\!\in\!\mathbb{R}^{d \times d}$ to produce $\mhsa\!\in\!\mathbb{R}^{N \times d}$. Self-attention explicitly models global interactions and is more flexible than grid-based operators (\eg convolutions) \cite{perez2019turing,cordonnier2019relationship}, but its quadratic cost in time and memory limits its applicability to high resolution images.

\paragraph{Spatially localizing self-attention.}

The global nature of self-attention directly conflicts with the spatial locality constraint of CAs; in response, we limit the connectivity structure of the attention operation to each cell's neighbourhood. This can be accomplished by either masking each head's attention matrix ($\mathbf{A}\!=\!\texttt{softmax}(\cdots) \in \mathbb{R}^{N \times N}$ in Eq.\ \ref{eq:sa}) with a banded matrix representing local connectivity (\eg \Fig{\ref{fig:overview}} \localize), or more efficiently,

\input{equations/localize_attn} Here, we assume top-left-to-bottom-right input flattening.
Instead of explicitly computing the global self-attention matrix $\mathbf{A}\!\in\!\mathbb{R}^{N \times N}$ then masking it, this approach circumvents the $\mathcal{O}(N^2d)$ computation in favour of an $\mathcal{O}(N\!M\!d)$ alternative that indexes the necessary rows and columns \emph{during} self-attention. The result is a localized self-attention matrix $\mathbf{A}^{\!\star}\!\in\!\mathbb{R}^{N \times M}$, where $M\!=\!N_HN_W\!\ll\!N$. As we show in our experiments, ViTCA is still capable of global self-attention despite its localization, by leveraging stored state information across cells and their global self-organization during CA iterations (\Fig{\ref{fig:teaser}}).

Following \mhsa\ is a multilayer perceptron (\Fig{\ref{fig:overview}} \mlp) with two layers and a GELU non-linearity. We apply Layer Normalization (LN) \cite{ba2016layer} before \mhsa\ and \mlp, and residual connections afterwards, forming a single encoding block. We use an MLP head (\Fig{\ref{fig:overview}} \mlphead) to decode to a desired output, with LN applied to its input, finalizing the ViTCA update rule $F_\theta$. In our experiments, ViT's \mlphead\ decodes directly into an image output whereas ViTCA decodes into update vectors added to cells.

\vspace{-.5\baselineskip}
\subsection{Update rule training procedure}
\vspace{-.5\baselineskip}
\label{subsec:update_rule}

To train the ViTCA update rule, we follow a ``pool sampling''-based training process \cite{palm2022variational,mordvintsev2020growing} along with a curriculum-based masking/noise schedule when corrupting inputs. During odd training iterations, we uniformly initialize a minibatch of cells \cells\ $\!=\!(\cellsplain_1,...,\cellsplain_b)$ with constant values (0.5 for output channels, 0 for hidden---see Appendix \ref{subsec:extended_ablation} for alternatives), then inject the masked input \maskedinput\ (see \Sec{\ref{subsec:denoising_autoencoding}}). After input injection, we asynchronously update cells ($\sigma\!=\!50\%$ update rate) using $F_\theta$ for $T\!\sim\!\mathcal{U}\{8,32\}$ recurrent iterations. We retrieve output \cellsoutput\ from the cell grid and apply an $L_1$ loss against the ground truth \gt. We also apply overflow losses to penalize cell output values outside of [0,1] and cell hidden values outside of [-1,1]. We use $L_2$ normalization on the gradient of each parameter in $\theta$. After backpropagation, we append the updated cells and their ground truths to a pool \pool\ which we then shuffle and truncate up to the first \poolsize\ elements. During even training iterations, we retrieve a minibatch of cells and their ground truths from \pool\ and process them as above. This encourages $F_\theta$ to guide cells towards a stable fixed-point. \Alg{\ref{alg:vitca_training}} in Appendix \ref{sec:appendix} details this process.

==> equations/losses.tex <==
\begin{equation}
  \begin{split}
    L_o &= \frac{1}{C_o}\|\mathbf{z}_o-\min(\max(\mathbf{z}_o, 0), 1)\|_1\ ,
    \\
    L_h &= \frac{1}{C_h}\|\mathbf{z}_h-\min(\max(\mathbf{z}_h, -1), 1)\|_1\ ,
    \\
    L_{rec} &= \frac{1}{C_o}\|\mathbf{z}_o - \mathbf{x}\|_1\ ,
    \\
    L &= \frac{1}{bHW}(\alpha L_{rec} + \beta(L_o + L_h))\ .
  \end{split}
  \label{eq:losses}
\end{equation}
